PatUntrack: Automated Generating Patch Examples for Issue Reports without Tracked Insecure Code

Security patches are essential for enhancing the stability and robustness of projects in the software community. While vulnerabilities are officially expected to be patched before being disclosed, patching vulnerabilities is complicated and remains a struggle for many organizations. To patch vulnerabilities, security practitioners typically track vulnerable issue reports (IRs), and analyze their relevant insecure code to generate potential patches. However, the relevant insecure code may not be explicitly specified and practitioners cannot track the insecure code in the repositories, thus limiting their ability to generate patches. In such cases, providing examples of insecure code and the corresponding patches would benefit the security developers to better locate and fix the insecure code. In this paper, we propose PatUntrack to automatically generating patch examples from IRs without tracked insecure code. It auto-prompts Large Language Models (LLMs) to make them applicable to analyze the vulnerabilities. It first generates the completed description of the Vulnerability-Triggering Path (VTP) from vulnerable IRs. Then, it corrects hallucinations in the VTP description with external golden knowledge. Finally, it generates Top-K pairs of Insecure Code and Patch Example based on the corrected VTP description. To evaluate the performance, we conducted experiments on 5,465 vulnerable IRs. The experimental results show that PatUntrack can obtain the highest performance and improve the traditional LLM baselines by +14.6% (Fix@10) on average in patch example generation. Furthermore, PatUntrack was applied to generate patch examples for 76 newly disclosed vulnerable IRs. 27 out of 37 replies from the authors of these IRs confirmed the usefulness of the patch examples generated by PatUntrack, indicating that they can benefit from these examples for patching the vulnerabilities.

==> algo/cok_hallu.tex <==
\begin{algorithm}[htbp]
\small
	%\SetAlgoNoLine %控制有无竖线
	\caption{Process of VulCoK.} 
 \label{alg:vulcok}
	\KwIn{The generated VTP description $\mathcal{G}_{VTP}=\{\mathcal{V}_{VTP},\mathcal{E}_{VTP}\}$, the external golden dataset $\mathcal{D}$.} 
	\KwOut{The corrected VTP description $\mathcal{G}_{VTP}'$.}
    \SetKwProg{Fn}{Function}{}{end}
    $Path\_Traverse \leftarrow\{Op_0\}$, $Next\_Traverse\leftarrow\{Op_0\}$, $\mathcal{G}_{VTP}'\leftarrow\mathcal{G}_{VTP}$\;\label{algo_line:traverse_start}
    \For {$OpItem \in Next\_Traverse$}{
        $Next\_Traverse = \{Op_i|{OpItem\rightarrow Op_i}\}$\;
        $Path\_Traverse\cap Next\_Traverse$\;
        \For {$OpConn \in Next\_Traverse$}{
            $GenQuery = LLM(\{OpItem, OpConn\}, P_{queryGen})$\;\label{algo_line:query_gen}
            Query $GoldenData$ with $GenQuery$ from $\mathcal{D}$\;
            $Type\_Detect, VTP\_Detect = LLM(\{OpItem, OpConn\}, \{OpItem\rightarrow OpConn\}, Path\_Traverse, GoldenData, P_{halDetect})$\;
            \If{$Type\_Detect=False$}{
            $OpItem.Vul\_Type = LLM(OpItem.Vul\_Type, P_{typeCorrect})$\;
             Go to line \ref{algo_line:query_gen}\;
            }
            \If{$VTP\_Detect=False$}{
             $\mathcal{G}_{VTP}'=LLM(\mathcal{G}_{VTP}',GoldenData, P_{vtpCorrect})$\;
            }               
        }
    }
    return $\mathcal{G}_{VTP}'$\;
    % \SetKwProg{Fn}{Function}{}{}
    % \Fn{AAA}{123} \tcc*[r]{AAA}
\end{algorithm}
% \vspace{-0.3cm}

==> tab/table_type_original.tex <==
\begin{table}[b]
\caption{The error types in the VTB operation nodes.}
\vspace{-0.2cm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|m{2.8cm}|m{5cm}}
\toprule
\textbf{ID} & \textbf{Error Types (VTP)}              & \multicolumn{1}{c|}{\textbf{Description}}                                                                                                                                                                            \\
\midrule
1 & Encoding \& Validation Errors        & The error comes from improperly handled, leading to unexpected behavior.                                   & Incompatible variable \& parameter \& return type \\
\arrayrulecolor{lightgray}\hline
2& \makecell[l]{Dependency \\ Errors}                        & The variables, functions, or libraries are unresolved or incorrect.    & Unbound name                                                                      \\
\hline
3&\makecell[l]{Injection \& Logic \\ Errors}                & The functions are improperly used leading to incorrect execution.             & Call error                                                                        \\
\hline
4&Memory Management \& Concurrency  Errors & The way how data is handled has errors, leading to exploitable conditions.                 & Incompatible attribute type, Unsupported operand                                  \\
\hline
5&Race \& Configuration Errors             & The error relates to the system conditions, affecting its correct operation.                             & Strengthened \& Weakened postcondition                                 \\
\hline
6&Buffer overflow                   & The error involves improper handling of boundaries and limits in data storage, leading to overflows or leaks. & Buffer overflow Errors                                                            \\
\hline
7&\makecell[l]{Error handling \\ \& logging issues}  & The encoding or decoding have errors, leading to XSS or injection attacks.                         & None\\
\arrayrulecolor{black}\bottomrule
\end{tabular}}
\vspace{-0.2cm}
\label{tab:error_types}
\end{table}
